FineSurE: Fine-grained Summarization Evaluation using LLMs

Automated evaluation is crucial for streamlining text summarization benchmarking and model development, given the costly and time-consuming nature of human evaluation. Traditional methods like ROUGE do not correlate well with human judgment, while recently proposed LLM-based metrics provide only summary-level assessment using Likert-scale scores. This limits deeper model analysis, e.g., we can only assign one hallucination score at the summary level, while at the sentence level, we can count sentences containing hallucinations. To remedy those limitations, we propose FineSurE, a fine-grained evaluator specifically tailored for the summarization task using large language models (LLMs). It also employs completeness and conciseness criteria, in addition to faithfulness, enabling multi-dimensional assessment. We compare various open-source and proprietary LLMs as backbones for FineSurE. In addition, we conduct extensive benchmarking of FineSurE against SOTA methods including NLI-, QA-, and LLM-based methods, showing improved performance especially on the completeness and conciseness dimensions. The code is available at https://github.com/DISL-Lab/FineSurE-ACL24.

==> floats/tab_bin.tex <==
\begin{table}[t]
\centering
\scalebox{0.88}{
\begin{tabular}{lccc}
\specialrule{0.1em}{0.2em}{0.2em}
Model & Original & Negation & Implicature \\
\hline
paraphrase            & 77.58                                                                & 82.41                                                                & 57.34                                                                   \\
IAE                   & 86.64                                                                & 79.63                                                                & 70.11                                                                   \\
instructor-base       & 89.06                                                                & 78.4                                                                 & 67.3                                                                    \\
instructor-large      & \textbf{89.59}                                                                & \textbf{87.38}                                                                & \textbf{73.54}                                                                  \\
\specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}
}
\caption{Binary classification.}
\label{tab:eval_res_bin}
\end{table}

==> floats/tab_challenges.tex <==
\begin{table*}[t]
    \centering
    \scalebox{0.95}{
    \begin{tabularx}{\textwidth}{thhh}
        \specialrule{0.1em}{0.2em}{0.2em} \\
        Intent & Original & Negation & Implicature \\
        \hline
        check timezone & I need to know britain's timezone & I don't need to know britain's timezone & I'm not sure when to start the event in Sydney \\
        set up timer & I need to start a timer & A timer started unexpectedly & I'm planning to do my workout every day at 6 am \\
        reserve restaurant & I'd like to make a reservation at rooth chris, can you do that & I mistakenly made a reservation at rooth chris, can you cancel that & Looking for a place to celebrate my friend's birthday with a large group \\
        why wrong exchange rate for card payment & I purchased something in a foreign currency but the rate applied is wrong & I purchased something in a foreign currency and the rate applied is correct & I've been noticing some discrepancies in my international transactions \\
        \specialrule{0.1em}{0.2em}{0.2em} \\
    \end{tabularx}}
    \caption{Examples of challenges.}
    \label{tab:prelim_exp}
\end{table*}

==> floats/tab_class.tex <==
\begin{table}[t]
\centering
\scalebox{0.86}{
\begin{tabular}{lcccc}
\specialrule{0.1em}{0.2em}{0.2em}
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{Implicature} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
                       & 0-shot       & 10-shot       & 0-shot         & 10-shot        \\
\hline
paraphrase             & 61.06        & 83.25         & 22.21          & 28.24          \\
IAE                    & 66.58        & 84.7          & 25.45          & 30.12          \\
instructor-base        & 67.48        & 85.77         & 26.18          & 30.88          \\
instructor-large       & \textbf{67.6}         & \textbf{86.2}          & \textbf{28.79}          & \textbf{34.26}         \\
\specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}
}
\caption{Classification.}
\label{tab:eval_res_class}
\end{table}

==> floats/tab_clus.tex <==
\begin{table}[t]
\centering
\scalebox{0.90}{
\begin{tabular}{lcccc}
\specialrule{0.1em}{0.2em}{0.2em}
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{Implicature} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
                            & KM    & Agg   & KM     & Agg     \\
\hline
paraphrase                  & 81.66      & 83.53           & 57.24       & 58.84             \\
IAE                         & 83.42      & 84.7            & 58.3        & 59.85             \\
instructor-base             & 83.82      & 84.89           & 57.93       & 59.18             \\
instructor-large            & \textbf{84.34}      & \textbf{86.01}           & \textbf{59.09}       & \textbf{61.35}    \\
\specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}
}
\caption{Clustering.}
\label{tab:eval_res_clus}
\end{table}

==> floats/tab_comparison_iae.tex <==
\begin{table*}[t]
\centering
\scalebox{0.684}{
\begin{tabular}{lccccccccccccccc}
\specialrule{0.1em}{0.2em}{0.2em}
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Triplet (ori)} & \multicolumn{2}{c}{Triplet (imp)} & \multicolumn{3}{c}{Binary Classification} & \multicolumn{2}{c}{Clustering (ori)} & \multicolumn{2}{c}{Clustering (imp)} & \multicolumn{2}{c}{Multi-class (ori)} & \multicolumn{2}{c}{Multi-class (imp)} \\
                       & T1              & T2              & T1              & T2              & Ori          & Neg          & Imp         & KM                & Agg              & KM                & Agg              & 0-shot            & 10-shot           & 0-shot            & 10-shot           \\ \hline
IAE                    & 25.34           & 84.90           & 3.51            & 68.11           & 87.29        & 79.98        & 70.52       & 83.43             & 84.63            & 61.89             & 64.20            & 66.31             & 84.52             & 25.53             & 30.41             \\
IAE-pos                & \cellcolor[HTML]{9AFF99} 27.74           & \cellcolor[HTML]{9AFF99} 85.81           & \cellcolor[HTML]{9AFF99} 4.35            & \cellcolor[HTML]{9AFF99} 68.88           & \cellcolor[HTML]{9AFF99} 87.83        & \cellcolor[HTML]{9AFF99} 80.91        & \cellcolor[HTML]{9AFF99} 70.85       & \cellcolor[HTML]{9AFF99} 83.63             & \cellcolor[HTML]{9AFF99} 84.96            & \cellcolor[HTML]{9AFF99} 62.09             & \cellcolor[HTML]{9AFF99} 64.54            & \cellcolor[HTML]{FFCCC9} 66.12             & \cellcolor[HTML]{FFCCC9} 84.36             & \cellcolor[HTML]{9AFF99} 26.20             & \cellcolor[HTML]{9AFF99} 30.91             \\
IAE-pos-neg            & \cellcolor[HTML]{9AFF99} 40.57           & \cellcolor[HTML]{9AFF99} 90.82           & \cellcolor[HTML]{9AFF99} 13.67           & \cellcolor[HTML]{9AFF99} 78.45           & \cellcolor[HTML]{9AFF99} 91.31        & \cellcolor[HTML]{9AFF99} 81.46        & \cellcolor[HTML]{9AFF99} 76.13       & \cellcolor[HTML]{FFCCC9} 82.95             & \cellcolor[HTML]{FFCCC9} 84.18            & \cellcolor[HTML]{9AFF99} 62.09             & \cellcolor[HTML]{FFCCC9} 65.14            & \cellcolor[HTML]{FFCCC9} 65.57             & \cellcolor[HTML]{FFCCC9} 84.41             & \cellcolor[HTML]{9AFF99} 25.64             & \cellcolor[HTML]{9AFF99} 30.55  \\
\specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}}
\caption{Adding LLM generated hard positive/negative to Intent-Aware-Encoder pre-training. Results averaged over $3$ random seeds.}
\end{table*}

==> floats/tab_hphnprompt.tex <==
\begin{table*}[t]
    \centering
    \scalebox{0.88}{
    \begin{tabularx}{\textwidth}{lsh}
        \specialrule{0.1em}{0.2em}{0.2em}
        Index & Prompt & Example \\
        \hline
        HP1 & ... Tell me 3 other kinds of [OBJECT] that you want to [ACTION] ... & what are the bike lanes like around the orlando area (know about,transportation) $\rightarrow$ interested in knowing about the public transportation system in orlando. \\
        HP2 & ... Give me 1 other ways to express what you want ... & can you still just recommend one please?? (be recommended,product) $\rightarrow$ can you please suggest a specific product or service that you think would be a good fit for me? \\
        HP3 & ... Give me 1 reasons that you want to do this ... & is highways 72 icy this morning? (know,weather) $\rightarrow$ could you help me know if the roads are icy so that i can take necessary precautions while driving. \\
        HP4 & ... Give me 2 things that you do not want to do in this scenario ... & remind me tomorrow to pick up charlie, pickup new glasses, grab groceries (be reminded,reminder) $\rightarrow$ i'd rather avoid forgetting to pick up charlie. \\
        HN1 & ... Give me 2 other things you want to [ACTION] rather than [OBJECT] ... & remind me tomorrow to pick up charlie, pickup new glasses, grab groceries (be reminded,reminder) $\rightarrow$ i want to be reminded to call my mom and wish her a happy birthday. \\
        HN2 & .. Now you no longer need to [ACTION] [OBJECT]. Give me 2 reasons for that ... & is highways 72 icy this morning? (know,weather) $\rightarrow$ i can check the weather forecast on my phone or computer. \\
        HN3 & ... Now you do not want to [ACTION] [OBJECT], give me 2 other things you want to do ... & when is my wakeup alarm on thursday (know,time) $\rightarrow$ want to know if there are any important events happening on thursday. \\
        \specialrule{0.1em}{0.2em}{0.2em} \\
    \end{tabularx}
    }
    \caption{Hard positive/negative utterance generation prompts.}
    \label{tab:train_data_prompt}
\end{table*}

==> floats/tab_human.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{c|c|c|c|c}
        \specialrule{0.1em}{0.2em}{0.2em}
        \multicolumn{3}{c}{Q1: convey intent?} & \multicolumn{2}{|c}{Q2: explicitly conveyed?} \\
        \hline
        original & negation & implicature & original & implicature \\
        \hline
        59 / 59 (100\%) & 9 / 59 (15.25\%) & 52 / 59 (88.14\%) & 46 / 52 (88.46\%) & 15 / 40 (37.50\%) \\
        \specialrule{0.1em}{0.2em}{0.2em}
    \end{tabular}
    \caption{Human evaluation breakdown.}
    \label{tab:eval_human_breakdown}
\end{table*}

==> floats/tab_main_large_dev.tex <==
\begin{table*}[t]
\centering
\scalebox{0.638}{
\begin{tabular}{lccccccccccccccc}
\specialrule{0.1em}{0.2em}{0.2em}
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Triplet (ori)} & \multicolumn{2}{c}{Triplet (imp)} & \multicolumn{3}{c}{Binary Classification} & \multicolumn{2}{c}{Clustering (ori)} & \multicolumn{2}{c}{Clustering (imp)} & \multicolumn{2}{c}{Multi-class (ori)} & \multicolumn{2}{c}{Multi-class (imp)} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} \cmidrule(lr){15-16}
                       & T1              & T2              & T1              & T2              & Ori          & Neg          & Imp         & KM                & Agg              & KM                & Agg              & 0-shot            & 10-shot           & 0-shot            & 10-shot           \\\hline
Baseline(14)               & 22.50            & 87.93           & 4.12            & 72.07           & 90.14        & 78.85        & 73.21       & 84.02             & 85.37            & 61.56             & 63.08            & 67.31             & 86.08             & 25.92             & 28.34             \\
Ours full(7)             & \cellcolor[HTML]{9AFF99}36.91           & \cellcolor[HTML]{FFCCC9}83.70            & \cellcolor[HTML]{9AFF99}12.57           & \cellcolor[HTML]{FFCCC9}55.95           & \cellcolor[HTML]{FFCCC9}73.87        & \cellcolor[HTML]{9AFF99}90.66        & \cellcolor[HTML]{FFCCC9}35.79       & \cellcolor[HTML]{9AFF99}84.57             & \cellcolor[HTML]{9AFF99}85.78            & \cellcolor[HTML]{9AFF99}64.24             & \cellcolor[HTML]{9AFF99}66.07            & \cellcolor[HTML]{9AFF99}69.85             & \cellcolor[HTML]{9AFF99}86.51             & \cellcolor[HTML]{9AFF99}27.69             & \cellcolor[HTML]{9AFF99}33.24             \\
-LLM(15)                  & \cellcolor[HTML]{9AFF99}41.79           & \cellcolor[HTML]{FFCCC9}87.15           & \cellcolor[HTML]{9AFF99}8.86            & \cellcolor[HTML]{FFCCC9}51.64           & \cellcolor[HTML]{FFCCC9} 89.09        & \cellcolor[HTML]{9AFF99}83.98        & \cellcolor[HTML]{FFCCC9} 53.52       & \cellcolor[HTML]{FFCCC9} 83.57             & \cellcolor[HTML]{FFCCC9} 84.35            & \cellcolor[HTML]{9AFF99}63.40              & \cellcolor[HTML]{9AFF99}65.42            & \cellcolor[HTML]{9AFF99}69.16             & \cellcolor[HTML]{FFCCC9} 85.53             & \cellcolor[HTML]{9AFF99}27.30              & \cellcolor[HTML]{9AFF99}32.05             \\
-HP(12)                   & \cellcolor[HTML]{9AFF99} 56.66           & \cellcolor[HTML]{9AFF99} 91.16           & \cellcolor[HTML]{9AFF99} 22.79           & \cellcolor[HTML]{FFCCC9} 64.79           & \cellcolor[HTML]{9AFF99} 90.65        & \cellcolor[HTML]{9AFF99} 85.05        & \cellcolor[HTML]{FFCCC9} 61.98       & \cellcolor[HTML]{FFCCC9} 80.59             & \cellcolor[HTML]{FFCCC9} 81.02            & \cellcolor[HTML]{9AFF99} 62.64             & \cellcolor[HTML]{9AFF99} 64.66            & \cellcolor[HTML]{FFCCC9} 66.35             & \cellcolor[HTML]{FFCCC9} 82.97             & \cellcolor[HTML]{FFCCC9} 25.81             & \cellcolor[HTML]{9AFF99} 30.31             \\
-HN(6)                   & \cellcolor[HTML]{FFCCC9} 16.71           & \cellcolor[HTML]{FFCCC9} 72.20            & \cellcolor[HTML]{FFCCC9} 3.07            & \cellcolor[HTML]{FFCCC9} 40.87           & \cellcolor[HTML]{FFCCC9} 58.89        & \cellcolor[HTML]{9AFF99} 89.68        & \cellcolor[HTML]{FFCCC9} 27.69       & \cellcolor[HTML]{9AFF99} 85.84             & \cellcolor[HTML]{9AFF99} 87.21            & \cellcolor[HTML]{9AFF99} 63.60              & \cellcolor[HTML]{9AFF99} 65.68            & \cellcolor[HTML]{9AFF99} 70.27             & \cellcolor[HTML]{9AFF99} 87.48             & \cellcolor[HTML]{9AFF99} 28.10              & \cellcolor[HTML]{9AFF99} 33.44             \\
-HP1(10)                                                      & \cellcolor[HTML]{9AFF99}36.02                         & \cellcolor[HTML]{FFCCC9} 82.92 & \cellcolor[HTML]{9AFF99} 12.04           & \cellcolor[HTML]{FFCCC9} 52.99           & \cellcolor[HTML]{FFCCC9} 68.27        & \cellcolor[HTML]{9AFF99} 92.03        & \cellcolor[HTML]{FFCCC9} 31.48       & \cellcolor[HTML]{9AFF99} 84.9              & \cellcolor[HTML]{FFCCC9} 85.28            & \cellcolor[HTML]{9AFF99} 65.65             & \cellcolor[HTML]{9AFF99} 67.60             & \cellcolor[HTML]{9AFF99} 73.36             & \cellcolor[HTML]{9AFF99} 87.05             & \cellcolor[HTML]{9AFF99} 33.88             & \cellcolor[HTML]{9AFF99} 36.65             \\
-HP2(9)                                                      & \cellcolor[HTML]{9AFF99} 37.41                         & \cellcolor[HTML]{FFCCC9} 82.78 & \cellcolor[HTML]{9AFF99} 13.11           & \cellcolor[HTML]{FFCCC9} 53.4            & \cellcolor[HTML]{FFCCC9} 70.76        & \cellcolor[HTML]{9AFF99} 90.87        & \cellcolor[HTML]{FFCCC9} 32.66       & \cellcolor[HTML]{9AFF99} 84.46             & \cellcolor[HTML]{FFCCC9} 85.08            &  \cellcolor[HTML]{9AFF99} 65.79             & \cellcolor[HTML]{9AFF99} 67.80             & \cellcolor[HTML]{9AFF99} 72.67             & \cellcolor[HTML]{9AFF99} 86.36             & \cellcolor[HTML]{9AFF99} 34.02             & \cellcolor[HTML]{9AFF99} 36.61             \\
-HP3(13)                                                      & \cellcolor[HTML]{9AFF99} 38.96                         & \cellcolor[HTML]{FFCCC9} 82.7  & \cellcolor[HTML]{9AFF99} 13.46           & \cellcolor[HTML]{FFCCC9} 53.23           & \cellcolor[HTML]{FFCCC9} 68.89        & \cellcolor[HTML]{9AFF99} 91.28        & \cellcolor[HTML]{FFCCC9} 32.92       & \cellcolor[HTML]{FFCCC9} 83.43             & \cellcolor[HTML]{FFCCC9} 84.54            & \cellcolor[HTML]{9AFF99} 65.24             & \cellcolor[HTML]{9AFF99} 66.63            & \cellcolor[HTML]{9AFF99} 72.47             & \cellcolor[HTML]{9AFF99} 86.30              & \cellcolor[HTML]{9AFF99} 33.26             & \cellcolor[HTML]{9AFF99} 35.36             \\
-HP4(8)                                                      & \cellcolor[HTML]{9AFF99} 54.79                         & \cellcolor[HTML]{9AFF99} 94.02 & \cellcolor[HTML]{9AFF99} 20.70            & \cellcolor[HTML]{9AFF99} 77.70            & \cellcolor[HTML]{9AFF99} 93.12        & \cellcolor[HTML]{9AFF99} 83.34        & \cellcolor[HTML]{FFCCC9} 72.16       & \cellcolor[HTML]{9AFF99} 84.17             & \cellcolor[HTML]{FFCCC9} 84.84            & \cellcolor[HTML]{9AFF99} 65.85             & \cellcolor[HTML]{9AFF99} 67.20             & \cellcolor[HTML]{9AFF99} 72.22             & \cellcolor[HTML]{9AFF99} 86.23             & \cellcolor[HTML]{9AFF99} 33.73             & \cellcolor[HTML]{9AFF99} 36.68             \\
-HP4-HN1(3)                                                  & \cellcolor[HTML]{9AFF99} 55.21                         & \cellcolor[HTML]{9AFF99} 94.72 & \cellcolor[HTML]{9AFF99} 21.13           & \cellcolor[HTML]{9AFF99} 79.3            & \cellcolor[HTML]{9AFF99} 94.23        & \cellcolor[HTML]{9AFF99} 82.51        & \cellcolor[HTML]{9AFF99} 77.15       & \cellcolor[HTML]{9AFF99} 84.81             & \cellcolor[HTML]{9AFF99} 85.46            & \cellcolor[HTML]{9AFF99} 66.49             & \cellcolor[HTML]{9AFF99} 67.79            & \cellcolor[HTML]{9AFF99} 72.73             & \cellcolor[HTML]{9AFF99} 86.98             & \cellcolor[HTML]{9AFF99} 33.90              & \cellcolor[HTML]{9AFF99} 36.92             \\
-HP4-HN2(11)                                                  & \cellcolor[HTML]{9AFF99} 32.39                         & \cellcolor[HTML]{FFCCC9} 85.96 & \cellcolor[HTML]{9AFF99} 6.29            & \cellcolor[HTML]{FFCCC9} 55.04           & \cellcolor[HTML]{FFCCC9} 86.61        & \cellcolor[HTML]{9AFF99} 86.61        & \cellcolor[HTML]{FFCCC9} 51.27       & \cellcolor[HTML]{9AFF99} 84.28             & \cellcolor[HTML]{FFCCC9} 85.17            & \cellcolor[HTML]{9AFF99} 65.65             & \cellcolor[HTML]{9AFF99} 67.53            & \cellcolor[HTML]{9AFF99} 72.63             & \cellcolor[HTML]{9AFF99} 86.60              & \cellcolor[HTML]{9AFF99} 33.42             & \cellcolor[HTML]{9AFF99} 36.20              \\
-HP4-HN3(5)                                                  & \cellcolor[HTML]{9AFF99} 52.44                         & \cellcolor[HTML]{9AFF99} 94.30  & \cellcolor[HTML]{9AFF99} 18.82           & \cellcolor[HTML]{9AFF99} 75.82           & \cellcolor[HTML]{9AFF99} 92.88        & \cellcolor[HTML]{9AFF99} 83.58        & \cellcolor[HTML]{FFCCC9} 71.12       & \cellcolor[HTML]{9AFF99} 85.20              & \cellcolor[HTML]{9AFF99} 85.95            & \cellcolor[HTML]{9AFF99} 65.71             & \cellcolor[HTML]{9AFF99} 67.68            & \cellcolor[HTML]{9AFF99} 73.21             & \cellcolor[HTML]{9AFF99} 86.78             & \cellcolor[HTML]{9AFF99} 33.08             & \cellcolor[HTML]{9AFF99} 36.91             \\
\cellcolor[HTML]{F9E79F} -HP4-HN1,3(1)     & \cellcolor[HTML]{9AFF99} 53.33                         & \cellcolor[HTML]{9AFF99} 94.88 & \cellcolor[HTML]{9AFF99} 20.84           & \cellcolor[HTML]{9AFF99} 78.42           & \cellcolor[HTML]{9AFF99} 93.88        & \cellcolor[HTML]{9AFF99} 82.28        & \cellcolor[HTML]{9AFF99} 73.94       & \cellcolor[HTML]{9AFF99} 84.65             & \cellcolor[HTML]{9AFF99} 86.65            & \cellcolor[HTML]{9AFF99} 66.18             & \cellcolor[HTML]{9AFF99} 68.32            & \cellcolor[HTML]{9AFF99} 73.51             & \cellcolor[HTML]{9AFF99} 87.78             & \cellcolor[HTML]{9AFF99} 34.24             & \cellcolor[HTML]{9AFF99} 37.64             \\
-HP1,4-HN1,3(2)   & \cellcolor[HTML]{9AFF99} 54.38                         & \cellcolor[HTML]{9AFF99} 94.48 & \cellcolor[HTML]{9AFF99} 20.52           & \cellcolor[HTML]{9AFF99} 76.40            & \cellcolor[HTML]{9AFF99} 93.26        & \cellcolor[HTML]{9AFF99} 83.32        & \cellcolor[HTML]{FFCCC9} 71.36       & \cellcolor[HTML]{9AFF99} 85.22             & \cellcolor[HTML]{9AFF99} 85.98            & \cellcolor[HTML]{9AFF99} 66.09             & \cellcolor[HTML]{9AFF99} 67.98            & \cellcolor[HTML]{9AFF99} 73.58             & \cellcolor[HTML]{9AFF99} 87.19             & \cellcolor[HTML]{9AFF99} 33.79             & \cellcolor[HTML]{9AFF99} 37.49             \\
-HP1,2,4-HN1,3(4) & \cellcolor[HTML]{9AFF99} 56.58                         & \cellcolor[HTML]{9AFF99} 94.16 & \cellcolor[HTML]{9AFF99} 21.75           & \cellcolor[HTML]{9AFF99} 75.34           & \cellcolor[HTML]{9AFF99} 93.24        & \cellcolor[HTML]{9AFF99} 83.48        & \cellcolor[HTML]{FFCCC9} 71.52       & \cellcolor[HTML]{9AFF99} 84.93             & \cellcolor[HTML]{9AFF99} 85.43            & \cellcolor[HTML]{9AFF99} 65.90              & \cellcolor[HTML]{9AFF99} 67.71            & \cellcolor[HTML]{9AFF99} 73.00                & \cellcolor[HTML]{9AFF99} 86.89             & \cellcolor[HTML]{9AFF99} 32.97             & \cellcolor[HTML]{9AFF99} 36.80              \\
\specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}}
\caption{Main results for instructor-large on dev set. Numbers in the brackets of first column are the rankings~\cite{colombo2022best}. \begin{tabular}{c} \cellcolor[HTML]{9AFF99}green\end{tabular} represents increased score and \begin{tabular}{c} \cellcolor[HTML]{FFCCC9}red\end{tabular} vice versa.}
\label{tab:exp_main_large_dev}
\end{table*}


==> floats/tab_main_large_test.tex <==
\begin{table*}[t]
\centering
\scalebox{0.65}{
\begin{tabular}{lccccccccccccccc}
\specialrule{0.1em}{0.2em}{0.2em}
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Triplet (ori)} & \multicolumn{2}{c}{Triplet (imp)} & \multicolumn{3}{c}{Binary Classification} & \multicolumn{2}{c}{Clustering (ori)} & \multicolumn{2}{c}{Clustering (imp)} & \multicolumn{2}{c}{Multi-class (ori)} & \multicolumn{2}{c}{Multi-class (imp)} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} \cmidrule(lr){15-16}
                       & T1              & T2              & T1              & T2              & Ori          & Neg          & Imp         & KM                & Agg              & KM                & Agg              & 0-shot            & 10-shot           & 0-shot            & 10-shot           \\\hline
Baseline               & 23.37           & 87.50           & 3.29            & 70.64           & 89.59        & 79.45        & \bf 73.87       & 84.34             & 86.01            & 62.22             & 64.36            & 67.60             & 86.20             & 29.23             & 34.12             \\
Disable LLM            & 39.26           & 86.20           & 7.99            & 50.83           & 89.18        & \bf 84.79        & 52.99       & 84.12             & 85.04            & 65.48             & 66.93            & 71.70             & 85.50             & 31.73             & 34.28             \\
Ours best              & \bf 51.13           & \bf 93.73           & \bf 20.35           & \bf 77.55           & \bf 94.04        & 83.10        & 73.56       & \bf 84.62             & \bf 86.75            & \bf 65.89             & \bf 68.21            & \bf 73.37             & \bf 87.24             & \bf 33.93             & \bf 37.16 \\ 
\specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}}
\caption{Main results for instructor-large on test set.}
\label{tab:exp_main_large_test}
\end{table*}

==> floats/tab_trip.tex <==
\begin{table}[t]
\centering
\scalebox{0.9}{
\begin{tabular}{lcccc}
\specialrule{0.1em}{0.2em}{0.2em}
\multirow{2}{*}{Model}     & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{Implicature} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & T1 & T2 & T1 & T2 \\
\hline
paraphrase       & 22.63                             & 84.76                             & \textbf{3.87}                                 & 68.92                                \\
IAE              & \textbf{24.04}                             & 84.26                             & 3.19                                 & 67.29                                \\
instructor-base  & 19.12                             & 86.09                             & 2.04                                 & 67.95                                \\
instructor-large & 23.37                             & \textbf{87.5}                              & 3.55                                 & \textbf{70.99}                         \\      
\specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}
}
\caption{Triplet task.}
\label{tab:eval_res_trip}
\end{table}

==> sections/copied-from-quip.tex <==
Automatic Evaluation for Dialogue Abstractive Summarization using LLM

PoC: Hwanjun Song, Hang Su

0. Summary

* We use closed-source LLM (Claude v2) for abstractive summarization evaluation, assessing different axes including general factuality, completeness, and conciseness.
* We introduced two reporting metrics to quantify the effectiveness: 
    * human-machine IAA score which measures agreement between human and machine annotations.
    * rank correlation which measures similarity between two model rankings derived from human and machine scores.
* On three benchmark datasets that have sentence-level annotations, we achieved human-machine IAA scores of 0.38 ~ 0.55 for general factuality and completeness, which are close to human-human IAA score. We observe rank correlation of 0.8+ on summaries generated by 4-6 summarization models.
* Prompt engineering helps improve the performance. chain-of-thought, evidence mapping, reasoning, adding task description, location of input conversation all contribute to the final result.

1. Motivation and Objective

Automated evaluation metric for abstractive summary is a must-need for efficient evaluation of summarization systems (e.g., different models, different prompts). It facilitates easy benchmarking and model development by providing information on whether the generated summaries meet our quality standard.

The existing automated metrics, e.g., Rouge and BERT-score, has been showing low correlation with real human judgement on the evaluation of summary quality. In this situation, LLMs has proven its potential to be as an automated tool for human-like evaluation [1, 2, 3]. In particular, G-Eval (using GPT-4) showed over 0.5 Spearman correlation coefficient with human likert scale judgement.

[1] Human-like Summarization Evaluation with ChatGPT
[2] G-Eval: NLG Evaluation using GPT-4 with Better Human Alignment
[3] Automatic Evaluation Using LLM [WIP] (Aura team’s effort)

Despite the availability of several LLM-based prompts, we chose to embark on our unique study to explore automated eval metrics, because:

* Our evaluation dimensions and granularities are different.
* We focus on dialogue input, not the news article (studied by existing works).
* We use anthropic models — Claude v2 (supported by Bedrock API), not the GPT-3.5 and GPT-4.
    * Our input is much longer than what previous works did (CNNDM).

2. Evaluation Dimensions 

Many dimensions were proposed for abstractive summary evaluation, but in this work we mainly focus on three key dimensions listed below:

Dimension	Explanation	Measurement
General factuality error *	This includes two types of sub-dimensions:

- Hallucination: summary content is not covered in the input transcript

- Non-hallucinatory factuality error: summary content is factually inconsistent with transcript, although mentioned in the input transcription	sentence-level
Completeness	- Model summary should include all key facts (as annotated by data team) of the input transcript.	summary-level
Conciseness	- The model summary should not have redundant sentences or mention information not in keyfact list.	summary-level

* We combine ‘hallucination’ and ‘non-hallucinatory factuality’ sub-dimensions into a single general factuality error in this research, as we find LLM cannot distinguish them between each other well.

Note that general factuality is annotated on sentence-level, whereas completeness and conciseness are summary-level metrics. To calculate completeness and conciseness, we need a keyfact list annotated by human, and then we compare summary sentences to keyfacts in the list. Annotation is thus done on keyfact-level, indicating whether each key fact is covered / linked to summary sentences. We call this annotation process “keyfact matching”, which is done by LLM in this work. The matching result can then be used to calculate summary-level completeness and conciseness.

3. Metrics for Automatic Evaluation

We present automated evaluation results, utilizing Inter-Annotator Agreement (IAA) scores that assess the agreement between human annotations and machine predicted annotations. 
In addition, we provide Rank Correlation, a measurement of similarity between two model rankings derived from human scores and machine scores, respectively. These rankings are determined by aggregating summary-level scores for each model. An example of ranking: model 1 > model 3 > model 2.

* IAA score between human and machine annotations (we used krippendorff alpha) :
    *  sentence-level factuality annotation
        * 0: sentence has no factual error, 1: sentence has factual error
    * keyfact matching annotation
        * 0: keyfact is not presented in the summary, 1:  keyfact is presented in the summary
* Rank correlation between human and machine scores (we used spearman correlation):
    * summary-level factuality score
        * Indicating percentage of factual sentences in the summary.
    * summary-level completeness score
        * Indicating percentage of key facts covered in the summary.
    * summary-level conciseness score
        * Indicating percentage of key sentences (summary sentence matched to key facts) in the summary.

4. Dataset exploration and  preparation

Selected benchmark datasets

Obtaining benchmark datasets is crucial for evaluating our proposed automatic metrics. We conducted a thorough examination on both internal and external benchmarks [link] and carefully selected three datasets that align with our evaluation dimensions.

Considerations for dataset selection: 

* IAA score among human annotators should be >= 0.4
* Has sentence-level factuality annotations
* Has human-annotated keyfact list

We chose the ‘Mediasum-2pass’ dataset as the benchmark for evaluating general factuality detection, and the ‘TCA-3pass-r1’ and ‘CL-refresh-2pass’ datasets for assessing completeness and conciseness dimensions, as follows:

Name	Creator	Base Data	Domain	Annotators
per Example	# examples	# sentences	# models for summary generation	Has sentence-level factuality labels?	Has human keyfact lists?	Evaluation Target
Mediasum-2pass (external data)	Liyan (our intern)	MediaSum	Interview	2 anno	171	476	6 models	Y	N	General factaulity
TCA-3pass-r1 (internal data)	CL data team	Meetings
Apptek
Rcc	sales call, meeting	3 anno	99	560	4 models	Y	Y	Completeness &
Conciseness
CL-refresh-2pass (internal data)	CL data team	Rcc-ks
Rcc-fin
Syntehtic-chat, ...	customer call	2 anno	123	454	4 models	Y	Y	Completeness &
Conciseness

Analysis on human IAA

Name	General Factuality Error	Key-fact matching
Mediasum-2pass (external data)	0.40	N/A
TCA-3pass-r1 (internal data)	0.19	0.51
CL-refresh-2pass (internal data)	0.34	0.62

5. Automatic evaluation for general factuality

Task definition:

Our objective is to determine whether sentences in the model summary contains any factuality error. This is represented by a binary annotation: ‘0 (no factuality error)’ and ‘1 (factuality error)’ for each sentence.

Input: 
Conversation, Summary sentences;

Output after XML parsing: 
A list of binary annotations for all summary sentences, e.g,. [0, 0, 1, 0];

Prompt design:

We tested over 10 different chain-of-thought prompts that integrate multiple design choices.

* explanation on factuality error types (e.g., out-of-context error, entity error)  → useful
* evidence mapping (detecting quotes related to the summary sentence) → useful
* reasoning of the determination → useful
* position of input inside the prompt (i.e., beginning, mid, end) → mid is the best
* we used XML output format as it exhibited better results than JSON format


See a detailed example of full input and output and results after XML parsing from our final prompt [here]

Evaluation on Mediasum-2pass using Best Prompt

We evaluate automatic evaluation results using human-machine IAA score and rank correlation. Human-human IAA score was improved from 0.28 to 0.38 by prompt tuning, which is close to human-human IAA score. Results are then accumulated to perform summary-level ranking.

Granularity	Sentence-level	Summary-level
Criteria	Human-Human IAA	Human-Machine IAA	Rank Correlation
Mediasum-2pass	0.40	0.38	0.83

Details on rank correlation: Model ranking is done based on summary-level general factuality scores. Predicted ranking is very similar to human ranking.

Type	chatgpt	wizardlm-30b	vicuna-7b	wizardlm-13b	claude	wizardlm-7b
Human eval 	1	2	3	4	5	6
Machine eval (prediction)	1	2	4	5	3	6

We also computed summary-level factuality error, which is the percentage of factual sentences in each summary. We see reasonable prediction scores, except in cases where the summaries are very poorly (wizardlm-7b).

Type	chatgpt	wizardlm-30b	vicuna-7b	wizardlm-13b	claude	wizardlm-7b
Human eval 	14%	25%	33%	34%	37%	61%
Machine eval (prediction)	14%	20%	29%	30%	23%	37%

6. Automated  evaluation on completeness and conciseness 

Task definition: keyfact matching

Keyfact matching is a task of checking if given human keyfacts are presented in the model summary. These results can be used to compute summary-level completeness and conciseness.

We ask LLMs to output a binary annotation for each keyfact: ‘0’ if a keyfact is not presented in the summary, or ‘1’ if a keyfact is covered in the summary. We also ask LLM to return the line number of summary sentences that are linked to the given keyfact.

Input: 
a list of human keyfacts, a model summary.

Output after XML parsing: 
a list of binary annotations for all key facts, e.g., [0, 0, 1, 1, 1]
a list of sentence ids in summary that are matched to keyfact lists, e.g., [1, 2, 4, 6]

Prompt engineering

Based on our analysis, we ended up using chain-of-thought, description of keyfact matching categories and evidence mapping to improve the performance.

See a detailed example of full input (prompt) and output, and results after XML parsing: [here]

Evaluation on TCA-3pass-r1 and CL-refresh-2pass

We evaluate human-machine IAA score and rank correlation on these two datasets. We observe high IAA scores comparable to human-human IAA for TCA-3pass-r1 (prompt was tuned on this data). 

		Keyfact Matching	Rank Correlation
Dataset		Human-human IAA	Human-Machine IAA	Completeness	Conciseness
TCA-3pass-r1	15%	0.51	0.55	0.80	1.00
CL-refresh-2pass		0.62	0.46	0.80	0.80

Details on rank correlation (TCA-3pass-r1 data): Model ranking is done based on summary-level completeness and conciseness. Results show similar rankings as compared to human judgement. There are only 4 models in this evaluation, so ranking is a less challenging task.

Dimension	Type	claudev1_instant-p10-4-7	claudev2-p11-2	titanL-p11-2	titanL-p10-4-7
Completeness	Human eval	1	2	3	4
Model prediction	2	1	3	4
Conciseness	Human eval 	1	2	3	4
Model prediction	1	2	3	4

On average summary-level completeness (%) and conciseness (%) per model, we see predicted scores similar to human scores.

Dimension	Type	claudev1_instant-p10-4-7	claudev2-p11-2	titanL-p11-2	titanL-p10-4-7
Completeness	Human eval	63.8%	60.8%	57.1%	35.8%
Machine eval (prediction)	65.6%	65.4%	64.6%	40.6%
Conciseness	Human eval	77.5%	62.5%	55.3%	51.0%
Machine eval (prediction)	76.4%	73.7%	63.1%	61.9%

7. Additional analysis on consistency and parsing success ratio

We compared our prompt with an existing work, and the results indicate that our prompt achieved 0.06 - 0.15 higher human-machine IAA scores. [see here]

Also, we conducted additional analysis on two major factors, which may affect the evaluation results [see here]

Consistency on prediction: Do the human-machine IAA results look differ with different runs?

* The results were not exactly the same but showed low variance for the three runs (0.01-0.03 difference in IAA)

Parsing success ratio: Since LLM is a generation model, the output of LLM may not follow our original design / prompt. Can the output of LLMs be parsed succesfully?

* Current prompts exhibited 93% for general factuality and 98-100% for completeness and conciseness.

8. Conclusion and Future Work

We proposed an automatic metric using Claude v2 to assess ‘general factuality’, ‘completeness’, and ‘conciseness’. Our experimental results demonstrated that our method achieved human-machine IAA scores on par with human-human IAA, along with a high rank correlation.

* Claude v2 generally shows reasonable evaluation performance on general factuality, completeness, and conciseness. 
* The acquisition of high quality data is crucial for LLM-based automatic evaluation. If the human-human IAA < 0.4, the LLM-based approach returns very low human-machine IAA.
* Complex prompts, which include evidence mapping, reasoning, and clear descriptions, yields better performance compared to simple ones.
* The placement of input transcript within the prompt impacts the final evaluation performance.
* XML format output shows slightly better performance than JSON format output.

Future work:

* Dataset: TCA-3pass and CL-refersh data exhibit low IAA scores for their general factuality annotation. It is important to enhance these datasets by revising our human annotation guidelines, thereby enabling effective utilization in the development of automated evaluation metric.
* Granularity: General factuality is a combination of ‘hallucination’ and ‘non-hallucinatory factuality error’. For a more accurate evaluation, we evaluate them separately.
* Keyfact generation: To evaluate completeness and conciseness, we necessitate a human keyfact list, indicating that our approach is not entirely automated. Moving forward, we should prioritize the development of keyfact generation methods.
* Improvement: For CL-refresh data, there is a room for further improvement on keyfact matching (human-human: 0.62, human-machine: 0.46)


Appendix A. Best Prompts

General factuality error:

Input: 


You will receive a transcript followed by a corresponding summary. 
Your task is to assess the factuality of each summary sentence across seven categories.

Out-of-Context Error: Content in the sentence is fabricated or is not explicitly mentioned by the transcript.
Predicate Error: A verb or predicate in the sentence is inaccurate or inappropriate compared to the transcript.
Entity Error: An essential component of a verb or predicate (e.g., subject, direct object, or indirect object) is erroneous when compared to the transcript.
Circumstantial Error: A circumstance presented in the sentence, usually through an adverbial phrase, is incorrect or misinterpreted when compared to the transcript.
Coreference Error: The sentence contains a verb or predicate that incorrectly refers to or represents an entity compared to the transcript.
Linking Error: The relationship between the meanings of two statements within the sentence is inaccurate or misinterpreted when compared to the transcript.
No Error: The sentence aligns explicitly with the content of the transcript and is factually consistent with it

Here is the transcript in <transcript></transcript> tags.
<transcript> 
LEMON : The coronavirus pandemic exacerbating issues facing the black community in the U.S. Issues like basic access to healthcare. Economic security and fair policing. I want to bring in now CNN's Van Jones and Dr. Camara Jones, an epidemiologist and family physician. Thank you both. Good to see both of you again. Van, I can't wait to see you for our special on Friday coming. So, Van, I'm going to start with you. Another black man shot dead broad daylight, another video. A family seeking justice at the same time, black Americans are getting pummeled by the coronavirus. Again, how much of this -- how much more of this can we take all at once? \nVAN JONES, CNN POLITICAL COMMENTATOR : You know, it's just horrible. You ask the question, what is it OK for us to do? What is it OK for a black man to do? You say, well, you know, we have poor underlying health conditions, it's our fault. You know, we should be in better health. OK, fine. Go jogging. Get in better health and then get killed. You say you have to wear a mask now. I have two teenage boys, they put on a mask, they take the mask off. I'm more afraid of somebody shooting them or arresting them for looking like quote and quote gang members than I'm afraid of this virus. What is it OK for us to do? What is allowed? We're crushed between police violence, vigilante violence. This virus. And anyway we move we feel trapped and nobody has an answer. You know, the last segment I just appreciate you, Don, for being able to hold that space. And for really starting this movement in the way you did. But is it very, very tough right now to be African-American in this situation. \nLEMON : Yes. Dr. Jones. You know, you have seen that disturbing video as a mom, what goes through your mind when you see a young black man out there jogging? I mean, today it would have been his 26th birthday. \nDR. CAMARA JONES, EPIDEMIOLOGIST AND FAMILY PHYSICIAN : Yes, he's just two years older than my son. And every time I see one of those videos then my first impulse is to call my son and say again, be careful. I worry about my husband going out in our neighborhood which is a predominantly white neighborhood at night to take the trash down to the street. And I say, well, let me do it. You know, it is our lives are not valued in this country. And our stories are not believed in this country. Our reality is not believed. Our voices are not heard. It's an invisibilization of our full humanity. \nJONES : I was talking to a -- \nLEMON : That plus -- hang on the one second. Let me get this in and you are going to -- that plus the pandemic. What is the impact to the African-American community aside from the sheer exhaustion of having to deal with these things? \nC. JONES : Well, I think that the impact is that we realize that our lives aren't valued by the meat packing plants. You know, our lives aren't valued or don't seem to be valued by these governors that are opening prematurely. That are essential roles have not been fully recognized or valued. Because we still don't have the PPE. We still don't have hazard pay. We still are not -- it's as if we are really, really, really seen as dispensable as animals. And what it reflects is white supremacist ideology. I'm just going to say one thing about that. White supremacist ideology is the idea that there's a hierarchy of human value with white folks at the top. And what we have in this country right now is that people at the top have said these are very fine people. These are good people. You know, encouraging people to bring out their -- I don't know if I want to say this. But I will just say that many of our leaders at the top are surrounding themselves with other people who have a vowed public white supremacist ideas. And so it's a signal to us that white supremacist flags has been waved is being heeded. \nLEMON : Yes. Van, I have to run. But I'll give you the last word. Quickly please, you have been in the seat. You know how that works, can you. \nJONES : Yes. I'll just say I was talking to a very prominent rapper today who said, he lives in a very wealthy neighborhood and he's afraid to leave his own house. He's spent all his money to live in a very wealthy neighborhood. But as an African-American young man he's afraid to leave his own house in that neighborhood for these reasons. \nLEMON : Thank you both. We are going to talk more and make sure you watch next Friday, when Van and I will host another special on the color of covid. That will be here at 10:00 p.m. on Friday. So make sure you tune in. We'll be right back.
</transcript>

Here are the sentences of the summary in <sentences></sentences> tags.
<sentences> 
Black Americans face disproportionate health and economic impacts from COVID-19 due to systemic racism.
Lack of healthcare, job security, and police violence threaten lives.
Leaders fail to value or protect black lives.
A prominent rapper fears leaving home in his wealthy neighborhood, showing injustice can affect anyone.
<sentences>

Instruction:
1. Compare each sentence within the <sentences></sentences> tags with the transcript.
2. Find exact quotes which can confirm the factual consistency of the sentence, and insert them in <quote></quote> XML tags. If you cannot, write \“not mentioned\” in the <quote></quote> XML tags.
3. Classify each sentence into one of the seven categories and provide a single sentence rationale of your classification within the <reason></reason> tags.
4. Write the classified category within the <type></type> tags.


Output:


Here are the annotated sentences:

<sentences>
<sentence>
Black Americans face disproportionate health and economic impacts from COVID-19 due to systemic racism.  <quote>
Our lives are not valued in this country. And our stories are not believed in this country. Our reality is not believed. Our voices are not heard. It's an invisibilization of our full humanity.
</quote>
<reason>
The quote supports the disproportionate impacts faced by Black Americans due to systemic racism.
</reason>
<type>No Error</type>
</sentence>

<sentence>
Lack of healthcare, job security, and police violence threaten lives.
<quote>not mentioned</quote>
<reason>The transcript does not explicitly mention lack of healthcare, job security, and police violence threatening lives.</reason>
<type>Out-of-Context Error</type> 
</sentence>

<sentence>
Leaders fail to value or protect black lives.
<quote>
It is as if we are really, really, really seen as dispensable as animals. And what it reflects is white supremacist ideology.
</quote>  
<reason>
The quote supports leaders failing to value black lives due to white supremacist ideology.
</reason>
<type>No Error</type>
</sentence>

<sentence>
A prominent rapper fears leaving home in his wealthy neighborhood, showing injustice can affect anyone.
<quote>
I was talking to a very prominent rapper today who said, he lives in a very wealthy neighborhood and he's afraid to leave his own house.
</quote>
<reason>
The quote directly supports the sentence's claims.
</reason>
<type>No Error</type>
</sentence>
</sentences>


Parsing XML Output:

pred_general_factuality_labels": [0.0, 1.0, 0.0, 0.0]



Keyfact matching:

You will receive a set of key facts and a summary for the same transcript.
Your task is to assess the inclusion of each key fact in the summary across three categories.

Precise Representation: The summary explicitly stated the key fact, and the fact is factually consistent with the summary.
Inaccurate Representation: The summary stated the key fact but contain inaccuracies or errors that need correction or clarification.
Omission: The summary does not mention the key fact at all.

Instruction:
1. Compare each key fact within the <key_facts></key_facts> tags with the summary.
2. Find the summary sentences which are pertaining to the key fact, and insert their line numbers separately in <lines></lines> XML tags. If you cannot, write \“not mentioned\” in the <lines></lines> XML tags.
3. Classify each key fact into one of the three categories and write the category within the <type></type> tags.

Here is the summary in <summary></summary> tags.
<summary>
[1] The conversation was about Turkey's role in the Middle East under Prime Minister Erdogan's government.
[2] While Turkey has had some issues domestically, it has played an increasingly positive role regionally.
[3] Turkey could serve as an economic model for countries like Egypt that are figuring out their path after revolution.
[4] Relations with Israel have been strained but could improve.
</summary>

Here are the key facts in <key_facts></key_facts> tags.
<key_facts>
According to the host, a recent presidential Republican debate described Turkey as a place where, under Prime Minister Recep Tayyip Erdogan, the murder rate against women has increased 1,400 percent; Washington Post columnist points out that Turkey's government amended its constitution to expand rights for women, ethnic minorities and unions
In Turkey press freedom has declined to the level of Russia.
Turkey's prime minister has embraced Hamas and threatened military force against both Israel and Cyprus.
The Erdogan government has been tougher on the armed wing of the Kurds, has carried out attacks on Iraq against that wings.
Turkey's relationship with Syria has also deteriorated, however Erdogan sent delegations there, declared that Syria was going to be a close ally of Turkey..
According to Washington Post columnist, Turkey has had a very rocky relationship with Israel and the threat to use force against Israel should not be taken seriously.
Turkey cannot improve its role in the rest of the Middle East and improve relations with Israel at the same time.
</key_facts>


Outputs:

<key_fact>
According to the host, a recent presidential Republican debate described Turkey as a place where, under Prime Minister Recep Tayyip Erdogan, the murder rate against women has increased 1,400 percent; Washington Post columnist points out that Turkey's government amended its constitution to expand rights for women, ethnic minorities and unions
</key_fact>
<lines>1, 2</lines>
<type>Precise Representation</type> 

<key_fact>
In Turkey press freedom has declined to the level of Russia.
</key_fact>
<lines>not mentioned</lines>
<type>Omission</type>

<key_fact>
Turkey's prime minister has embraced Hamas and threatened military force against both Israel and Cyprus.
</key_fact>
<lines>not mentioned</lines>
<type>Omission</type>

<key_fact>
The Erdogan government has been tougher on the armed wing of the Kurds, has carried out attacks on Iraq against that wings.
</key_fact>
<lines>not mentioned</lines>
<type>Omission</type>

<key_fact>
Turkey's relationship with Syria has also deteriorated, however Erdogan sent delegations there, declared that Syria was going to be a close ally of Turkey..
</key_fact>
<lines>not mentioned</lines>
<type>Omission</type>

<key_fact>
According to Washington Post columnist, Turkey has had a very rocky relationship with Israel and the threat to use force against Israel should not be taken seriously.
</key_fact>
<lines>4</lines>
<type>Precise Representation</type>

<key_fact>
Turkey cannot improve its role in the rest of the Middle East and improve relations with Israel at the same time.
</key_fact>
<quote>not mentioned</quote>
<type>Omission</type>


Parsing XML Output:

Predicted key-fact matching labels = [1, 0, 0, 0 ,0 ,1 ,0]
Line numbers of matched sentences = [1, 2, 4]


Computed summery-level completeness and conciseness:

completeness = 2 (# matched keyfacts) / 7 (# total keyfacts)
conciseness = 3 (# key sentences) / 4 (# all sentences in summary)



Appendix B. Calculation of completeness and conciseness score using keyfact matching

* Summary-level completeness 
    Measuring percentage of key facts covered in the summary.
    (# of matched human keyfacts / total # of human key facts) 
* Summary-level conciseness:
    Measuring percentage of key sentences (summary sentence matched to key facts) in the summary .
    (# of matched summary sentences / total # of summary sentences)



Appendix C. Additional Analysis

Comparison with existing work

We compared our prompt with the one proposed by “Human-like Summarization Evaluation with ChatGPT [link]. The baseline prompts are described here.

We only report IAA scores, since the baseline prompt is not designed for getting rank correlation.

* IAA for general factuality: our prompt shows an IAA score that is 0.15 higher.

Data	Human-Human IAA	Human-Machine IAA (baseline)	Human-Machine IAA (ours)
Mediasum-2pass	0.40	0.23	0.38

* IAA for completeness and conciseness: our prompt shows IAA scores that are 0.08 and 0.06 higher for two datasets, respectively.

Data	Human-Human IAA	Human-Machine IAA (baseline)	Human-Machine IAA (ours)
TCA-3pass-r1	0.51	0.47	0.55
CL-refresh-2pass	0.62	0.40	0.46

Consistency check

We conducted three tests to evaluate general factuality. The results are not exactly the same but show low variance for the three runs.

* General factuality eval on Meidasum-2pass data

Method	Human-Machine IAA	Rank Correlation
Run 1	0.38	0.83
Run 2	0.37	0.77
Run 3	0.36	0.77

* Keyfact matching eval on TCA-3pass-r1 data

Method	Human-Machine IAA	Rank Correlation (Completeness)	Rank Correlation (Conciseness)
Run 1	0.55	0.80	1.00
Run 2	0.56	1.00	0.80
Run 3	0.53	1.00	1.00

Parsing success ratio

Although we prompted the LLM to output a specific format (i.e., XML in this case), the LLM potentially produces output that is not able to parse, resulting in inconsistent results due to different level of parsing error.

* The LLM returns entirely wrong format, e.g., wrong XML format like missing close tags, or tag ordering issue.
* The LLM returns correct format but there is a mismatch in the number of key fact matching labels between predictions and human key-facts (see the example)


Fortunately, Claude v2 shows over 90% parsing success ratios.

Measurement	Dataset	Parsing success ratio
General factuality	Mediasum-3pass	93%
Completeness & Conciseness	TCA-3pass-r1	98%
CL-refresh-2pss	100%



==> sections/lim.tex <==
\section*{Limitations}\label{sec:lim}

In this paper, we used ChatGPT for evaluation and a smaller LLM \texttt{falcon-40b-instruct} for training. This is mainly due to the legal concern. Our use of OpenAI for this publication, is to the best our knowledge, in compliance with applicable OpenAI’s terms and conditions as of March 14, 2023. However, we argue that using a larger and more capable LLM can potentially improve the quality of data generated and thus further improve the model.
